Spectral Surgery: Training-Free Refinement of LoRA via Gradient-Guided Singular Value Reweighting

Low-Rank Adaptation (LoRA) improves downstream performance by restricting task updates to a low-rank parameter subspace, yet how this limited capacity is allocated within a trained adapter remains unclear. Through a geometric and empirical study across multiple tasks and backbones, we find that trained LoRA updates often exhibit an inefficient spectrum: task effects concentrate in a small subset of singular directions, while many remaining components are neutral or detrimental, motivating post-hoc refinement within the learned subspace. We propose Spectral Surgery, a training-free refinement that decomposes a LoRA update with SVD, estimates per-component sensitivity using gradients on a small calibration set, and reweights singular values under a magnitude constraint while keeping the learned directions fixed. Across Llama-3.1-8B and Qwen3-8B on four benchmarks, Spectral Surgery yields consistent gains (up to +4.4 points on CommonsenseQA and +2.4 pass@1 on HumanEval) by adjusting only $\approx 1{,}000$ scalar coefficients. These results demonstrate that SVD-structured, low-cost parameter editing can serve as a practical route to improving trained LoRA adapters in a purely post-hoc manner.

==> new_intro0128.tex <==
Low-Rank Adaptation (LoRA) has become the de facto standard for task-specific adaptation of large language models (LLMs) due to its strong empirical performance and favorable efficiency profile: instead of updating the full weight space, LoRA injects a low-rank update $\Delta W$ into selected linear layers while keeping the backbone frozen \citep{hu2022lora}. In practice, a LoRA adapter is often treated as a static endpoint of training: once optimization converges, the resulting low-rank matrix is deployed as-is, and rarely revisited.

This “train-then-freeze” convention hides a natural question. From the task-vector view of adaptation, a trained adapter is a compact representation of a task-induced displacement in parameter space \citep{ilharco2023editing}. Yet convergence of SGD does not guarantee that the limited representational budget of a rank-$r$ update is used efficiently: even within a fixed low-rank subspace, different internal allocations can encode dramatically different behaviors. This raises a basic efficiency gap that is orthogonal to choosing a larger rank or a better training recipe: \emph{given a converged LoRA adapter, is the capacity inside its learned rank being allocated in the most useful way?}

To study this question, we analyze trained LoRA updates through their spectral structure. Writing the LoRA update as $\Delta W = BA$ and computing the thin SVD of the resulting product matrix yields
$\Delta W = U \Sigma V^\top$,
where $U$ and $V$ define a rank-$r$ singular subspace and $\Sigma$ specifies the energy distribution across the $r$ components. Our geometric analysis reveals a striking dichotomy between these two ingredients. In residual-writing projections---notably the attention output projection and the MLP down projection ---the learned singular subspaces exhibit strong alignment across layers and even across module types. Empirically, we observe a layer-invariant ``backbone'' in which within-layer output- and down-projection updates coordinate on a shared residual feature subspace (Figure~\ref{fig:align_intra}). This suggests that optimization is comparatively reliable at discovering task-aligned directions.

In contrast, the singular values---the spectrum that allocates energy across those directions---often appear far less ``well-behaved.'' Within an already-aligned subspace, $\Sigma$ may over-amplify components that do not translate into downstream capability, while under-amplifying components that are genuinely useful. Put differently, even when the adapter has found the right task-aligned directions, it may assign the wrong spectral weights. This motivates a hypothesis: the bottleneck for many trained LoRA adapters is not only the rank itself, but the \emph{spectral efficiency} of how energy is distributed within the learned rank.

Existing work that touches LoRA’s structure largely falls into two regimes.
Training-time interventions improve low-rank adaptation by modifying how the adapter is learned---e.g., changing optimization dynamics, reallocating rank/budget, or shaping initialization via decomposition---which can yield better adapters but necessarily requires re-training and does not answer how to improve an already-converged $\Delta W$ \citep{hayou2024loraplus,zhang2023adalora,meng2024pissa,corda2025}.
In parallel, diagnostic analyses use spectral or geometric lenses to reveal qualitative structure and potential pathologies in low-rank updates (e.g., spurious or harmful components, or differences from full fine-tuning), but typically stop at interpretation rather than providing an actionable correction mechanism \citep{shuttleworth2024lora,bidermanlora}.
As a result, a practical middle ground remains underexplored: \emph{post-training refinement}---a lightweight procedure that treats a trained adapter as an editable object and improves it after convergence, under explicit structural constraints.

Based on this insight, we propose \textbf{Spectral Surgery}, a training-free, post-hoc refinement framework for LoRA adapters.
The core principle is simple: \emph{keep the subspace, fix the spectrum}.
Concretely, we preserve the learned singular directions to maintain the observed geometric alignment, and only modulate the singular-value spectrum to reallocate energy within the fixed rank budget.
Our edits are guided by a small calibration set: we estimate which spectral components are most sensitive to the target objective and selectively rescale them---amplifying under-utilized task-relevant components while suppressing components that behave like noise---under conservative magnitude/energy constraints.
This refinement touches only $O(r)$ scalars per edited module (often $\approx 10^3$ in total) and requires no further training.

We evaluate Spectral Surgery on two 8B backbones (Llama-3.1-8B~\citep{Dubey2024TheL3} and Qwen3-8B~\citep{Yang2025Qwen3TR}) across reasoning, coding, and instruction-following benchmarks. Spectrum-only editing yields clear but task- and model-dependent improvements. For example, on CommonsenseQA~\citep{commonsenseqa} with Llama-3.1-8B, sensitivity-guided spectrum modulation improves accuracy by approximately $+4.2$--$+4.4$ absolute points over the unedited adapter; on Qwen3-8B, we observe improvements up to $+4.2$ points in HumanEval~\citep{chen2021evaluating} pass@1 under the same post-hoc editing principle. These gains are achieved while adjusting orders of magnitude fewer degrees of freedom than even a small additional fine-tuning run.

Crucially, our analysis includes a random-index control, where sensitivity scores are randomly mapped to spectral components. We find that randomized perturbations can sometimes outperform the unedited baseline. Rather than undermining our method, this diagnoses a critical pathology: standard LoRA training often results in \emph{spectral overfitting}, where the spectrum is so brittle that even unstructured regularization (random noise) brings improvements. Spectral Surgery unifies this view: it acts as a robust regularizer when sensitivity signals are noisy, and as a precise signal amplifier when calibration data is reliable. This also implies that post-hoc editing requires task-aware validation, as objective mismatch (e.g., in strict instruction following) can lead to degradation if not constrained.


In summary, our contributions are: 
\begin{enumerate} 
\item \textbf{Perspective:} We uncover the subspace--spectrum dichotomy in trained LoRA adapters, identifying spectral inefficiency as a primary post-training bottleneck. 
\item \textbf{Method:} We propose Spectral Surgery, a training-free framework that refines adapter capability by selectively reweighting singular values based on calibration sensitivity. 
\item \textbf{Findings:} We demonstrate that spectrum-only editing provides clear performance gains and, through random controls, characterizes the ``brittleness" of standard LoRA solutions. 
\end{enumerate}


==> old_abs.tex <==
Low-Rank Adaptation (LoRA) has become ubiquitous for LLM fine-tuning, yet the spectral efficiency of the learned update matrices remains underexplored. We identify that standard LoRA training often results in a sub-optimal mixture of task-critical signals and optimization noise within the singular value spectrum. To address this, we propose a tuning-free spectral editing framework that refines pre-trained adapters using gradient-based sensitivity analysis on a minimal calibration set. By selectively scaling singular values—amplifying high-sensitivity components while suppressing noise—we perform precise "surgery" on the model weights without further training. Empirical results on Llama series across reasoning (GSM8K) and coding (HumanEval) benchmarks demonstrate consistent performance gains (e.g., ~1\% absolute improvement), achieved by adjusting fewer than 1,000 scalar parameters. This work highlights the critical role of spectral disentanglement in maximizing the capacity of parameter-efficient adapters beyond their initial convergence.

==> old_intro.tex <==


A useful lens for understanding adaptation in large language models (LLMs) is the \emph{task vector} view: fine-tuning induces a parameter displacement $\Delta\theta$ that can be treated as a direction encoding task-specific behavior, enabling arithmetic operations such as addition/subtraction across tasks \citep{ilharco2023editing}. From this perspective, editing a model can be cast as editing a task vector—either by composing multiple task vectors or by transforming a single task vector to better align with downstream objectives.

LoRA offers a parameter-efficient instantiation of this idea. Instead of a dense $\Delta\theta$, LoRA injects structured low-rank updates $\Delta W$ into frozen layers \citep{hu2022lora}. However, the prevailing paradigm still treats a trained LoRA adapter as a static endpoint: once training concludes, the learned update is rarely inspected or \emph{edited}. This is a missed opportunity, because even a low-rank task vector has internal structure—most notably its \emph{spectral decomposition}. Recent analyses suggest that LoRA and full fine-tuning can exhibit qualitatively different spectral signatures, with LoRA occasionally allocating capacity into directions that are suboptimal for the target task \citep{shuttleworth2024lora}. Moreover, LoRA can lag behind full fine-tuning on specialized benchmarks despite preserving general capabilities \citep{biderman2024lora}, hinting that part of the gap may come from how spectral mass is distributed within the learned low-rank update.

In this work, we propose to treat a trained LoRA adapter as an explicit \emph{task vector} that can be \emph{edited post hoc}. Our key hypothesis is that a learned low-rank update $\Delta W$ mixes task-critical components with redundant—or potentially deleterious—components, and that re-allocating spectral mass \emph{within the same learned subspace} can improve downstream performance without retraining. This view connects naturally to model editing: instead of injecting new knowledge or rewriting base weights, we perform a structured edit on the adapter's task vector with strong constraints that preserve parameter efficiency.

We introduce \textbf{LoRA-Spectral-Edit}, a lightweight procedure that:
(i) decomposes each LoRA update $\Delta W$ via SVD;
(ii) estimates the task sensitivity of each singular direction using gradient projections on a small calibration set; and
(iii) applies a spectrum-only edit by reweighting singular values while preserving singular vectors.
% Our procedure is agnostic to how an adapter is obtained, and applies broadly to \emph{LoRA-family} adapters (including popular variants such as LoRA+~\citep{hayou2024loraplus}, PiSSA~\citep{meng2024pissa}, and AdaLoRA~\citep{zhang2023adalora}) by operating directly on the realized low-rank update $\Delta W$.
We evaluate LoRA-Spectral-Edit on four representative capabilities:
\textbf{mathematical reasoning} (trained on MetaMathQA~\citep{yu2023metamath}, evaluated on GSM8K~\citep{cobbe2021training}),
\textbf{code generation} (trained on Magicoder~\citep{wei2023magicoder}, evaluated on HumanEval~\citep{chen2021evaluating}),
\textbf{instruction following} (trained on Alpaca~\citep{alpaca}, evaluated on IFEval~\citep{ifeval}), and
\textbf{commonsense reasoning} (trained on CommonsenseQA~\citep{commonsenseqa}, evaluated on CommonsenseQA~\citep{commonsenseqa}).


Across two 8B backbones (Llama-3.1-8B and Qwen3-8B) and four benchmarks, LoRA-Spectral-Edit yields clear but \emph{task- and model-dependent} effects.
On \textbf{CommonsenseQA} with \textbf{Llama-3.1-8B}, \texttt{grad\_direction} delivers the largest and most consistent gains: accuracy improves by \textbf{+0.042--0.044} over the unedited adapter across calibration sizes 64--256 (e.g., $0.740\!\rightarrow\!0.784$).
On \textbf{Qwen3-8B}, \texttt{grad\_direction} provides modest improvements on \textbf{GSM8K} (up to \textbf{+0.009}, $0.808\!\rightarrow\!0.817$) and stronger gains on \textbf{HumanEval} (up to \textbf{+0.042} pass@1, $0.488\!\rightarrow\!0.530$), while changes on \textbf{CSQA} are small (typically $\le$ \textbf{+0.007}).
For \textbf{IFEval}, spectrum-only reweighting yields small improvements on \textbf{Llama-3.1-8B} (best \textbf{+0.018}, $0.305\!\rightarrow\!0.323$), whereas on \textbf{Qwen3-8B} the best scores come from the \texttt{random\_index} control (\textbf{+0.007--0.016}) and \texttt{grad\_direction} can fail catastrophically (dropping to $\sim$0.17--0.18), underscoring the need for task-aware validation and safe fallbacks.




Our contributions are: \lz{贡献一般只列3点}
\begin{itemize}
    \item \textbf{Framing:} We cast a trained LoRA adapter as a \emph{structured task vector} and study \emph{post-hoc task-vector editing} constrained within its learned low-rank subspace.
    \item \textbf{Method:} We propose a lightweight, training-free editing framework that performs \emph{spectrum-only} updates to $\Delta W$ (reweighting singular values while preserving singular vectors), guided by a gradient-projection sensitivity signal computed on a small calibration set.
    \item \textbf{Evaluation:} We run controlled comparisons across two 8B backbones, four benchmarks, and multiple calibration sizes, including a \texttt{random\_index} control to separate signal from incidental changes. Empirically, sensitivity-guided edits produce \textbf{large and consistent} gains on Llama-3.1-8B CommonsenseQA (\textbf{+0.042--0.044} acc), and \textbf{moderate} improvements on Qwen3-8B for GSM8K (up to \textbf{+0.009} acc) and HumanEval (up to \textbf{+0.042} pass@1), but also expose \textbf{clear failure modes} (e.g., \texttt{grad\_direction} on Qwen3-8B IFEval), highlighting that the reliability of the sensitivity signal is task-dependent and requires validation/fallback mechanisms.
\end{itemize}




==> old_setup.tex <==
\section{Experimental Setup}
\label{sec:exp_setup}

\subsection{Benchmarks and Metrics}
We evaluate spectrum-only adapter editing across four capabilities. For each capability, we train an adapter on a task-specific corpus and evaluate on a downstream benchmark using \texttt{lm\_eval} with the \texttt{vllm} backend.

\begin{itemize}
    \item \textbf{Mathematical reasoning:} train on \textsc{MetaMath}, evaluate on \textsc{GSM8K}. We report \textbf{accuracy} (the harness reports \texttt{acc} / \texttt{exact\_match}; we use \texttt{acc} as the primary key).
    \item \textbf{Code generation:} train on \textsc{Magicoder}, evaluate on \textsc{HumanEval} . We report \textbf{pass@1} from the harness.
    \item \textbf{Instruction following:} train on \textsc{Alpaca}, evaluate on \textsc{IFEval} . We report the benchmark-defined \textbf{strict instruction-following accuracy} (we prioritize \texttt{prompt\_level\_strict\_accuracy} when available).
    \item \textbf{Commonsense reasoning:} train on \textsc{CommonsenseQA}, evaluate on \textsc{CommonsenseQA} . We report \textbf{accuracy}.
\end{itemize}

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{l l l l}
% \toprule
% \textbf{Capability} & \textbf{Train} & \textbf{Eval} & \textbf{Metric (lm\_eval)} \\
% \midrule
% Math & MetaMath & GSM8K & acc  $\uparrow$ \\
% Code & Magicoder & HumanEval & pass@1  $\uparrow$ \\
% Instr. follow & Alpaca & IFEval & prompt\_level\_strict\_accuracy  $\uparrow$ \\
% Commonsense & CSQA & CSQA & acc  $\uparrow$ \\
% \bottomrule
% \end{tabular}
% \caption{Tasks and evaluation metrics.}
% \label{tab:tasks_metrics}
% \end{table}
\subsection{Base Models}
We consider two widely used 8B-class decoder-only LLMs:
\textbf{Llama-3.1-8B} and \textbf{Qwen3-8B}.
All adapters are trained and evaluated on the same base model they were trained from; our edits do not modify base weights.

\subsection{Training Protocol}
To make comparisons controlled, we standardize training across adapter types as much as possible.
We use the same optimizer family, batch construction, max sequence length, and data preprocessing per task.
Unless noted otherwise, we:
(i) train each adapter for a fixed number of epochs $E$ (default $E=3$);
(ii) for large training corpora, cap the number of training examples to a fixed budget (we use $50$k in our main runs for MetaMath/Magicoder) to keep compute comparable across tasks;
and (iii) run multiple random seeds and report mean$\pm$std (Sec.~\ref{sec:motivation}).

\paragraph{Target modules.}
Adapters are trained on a standard set of Transformer projection modules (attention and MLP).
However, \emph{editing} is restricted to residual-writing modules
\texttt{o\_proj} and \texttt{down\_proj} (Sec.~\ref{sec:motivation}),
since these share the residual output space and exhibit strong subspace alignment (Fig.~\ref{fig:alignment_analysis}).

\subsection{Calibration Data for Sensitivity Estimation}
To estimate per-singular-direction sensitivity, we use a small \emph{calibration} set $\mathcal{D}$ drawn from the same training distribution of the adapter (and disjoint from evaluation sets).
In our implementation, we use $n_{\text{cal}}=32$ examples by default (batch size $2$) and aggregate sensitivities with a mean-absolute reducer (corresponding to the \texttt{mean\_abs} option in our editing CLI):
\begin{equation}
s_k \;=\; \frac{1}{n_{\text{cal}}}\sum_{i=1}^{n_{\text{cal}}}\left|u_k^\top G^{(i)} v_k\right|.
\end{equation}
Unless otherwise specified, we use a fixed calibration seed and do not shuffle the calibration set; shuffling and alternative reducers are ablated in Sec.~\ref{sec:ablations_calib}.
\subsection{Editing Protocol and Hyperparameters}
We apply spectrum-only edits per module and per layer, preserving $U,V$ and modifying only $\sigma$:
\begin{equation}
\Delta W' = U\,\mathrm{diag}(\sigma')\,V^\top,\qquad \sigma'_k=\alpha_k\sigma_k.
\end{equation}
In the evaluation pipeline, we run four edit policies:
\texttt{abs\_select}, \texttt{smooth\_abs}, \texttt{random\_index} (control), and \texttt{grad\_direction}.

\paragraph{Default hyperparameters (implementation).}
For \texttt{abs\_select} and \texttt{random\_index}, we use \texttt{core\_frac}=0.2, \texttt{noise\_frac}=0.2, $\gamma_{\text{amp}}=1.25$, $\gamma_{\text{sup}}=0.80$.
For \texttt{smooth\_abs}, we use \texttt{smooth\_temperature}=0.35, \texttt{smooth\_center\_q}=0.5, with the same $(\gamma_{\text{amp}},\gamma_{\text{sup}})$.
For \texttt{grad\_direction}, we use multiplicative updates with an asymmetric rule (\texttt{eta\_suppress}=2.0, \texttt{eta\_enhance}=0.2).

\paragraph{Magnitude control.}
By default, we preserve $\ell_1$ spectral mass (the \texttt{preserve\_energy=l1} option in our implementation), preventing trivial gains caused by global rescaling.
\subsection{Evaluation Protocol}
\label{sec:eval_protocol}
We fix evaluation procedures to isolate the effect of editing. All evaluations are executed via \texttt{lm\_eval} using the \texttt{vllm} backend with \texttt{dtype=auto}, \texttt{batch\_size=auto}, and tensor parallelism (default: 8-way).
When evaluating an adapter, we either load it through vLLM's LoRA interface (\texttt{lora\_local\_path}, with \texttt{max\_lora\_rank} read from the adapter config) or, if needed, merge it into the base model offline for robustness.

\begin{itemize}
    \item \textbf{GSM8K (\texttt{gsm8k}):} 5-shot evaluation with deterministic decoding (\texttt{temperature=0, top\_p=1}). We report the harness accuracy metric (primary key: \texttt{acc}).
    \item \textbf{HumanEval (\texttt{humaneval}):} 0-shot evaluation with deterministic decoding (\texttt{temperature=0, top\_p=1}). We enable code execution in the harness (\texttt{--confirm\_run\_unsafe\_code} and \texttt{HF\_ALLOW\_CODE\_EVAL=1}) and report \texttt{pass@1}.
    \item \textbf{IFEval (\texttt{ifeval}):} evaluation with the harness default protocol, using \texttt{max\_gen\_toks=2048} and deterministic decoding (\texttt{temperature=0, top\_p=1}). We report strict instruction-following accuracy (primary key: \texttt{prompt\_level\_strict\_accuracy} when available).
    \item \textbf{CommonsenseQA (\texttt{commonsense\_qa}):} 0-shot multiple-choice evaluation under the harness formatting; we report \texttt{acc}.
\end{itemize}



==> tables/all_data.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{l c l l c c c c c}
\toprule
\textbf{Model} & \textbf{Calib} & \textbf{Task} & \textbf{Metric} &
\textbf{Baseline} & \textbf{abs\_select} & \textbf{smooth\_abs} & \textbf{random\_index} & \textbf{grad\_direction} \\
\midrule
Llama-3.1-8B & 32 & GSM8K & acc & \textbf{0.668} & 0.657 & 0.660 & 0.657 & 0.622 \\
Llama-3.1-8B & 32 & HumanEval & pass@1 & \textbf{0.494} & \textbf{0.494} & 0.476 & 0.488 & 0.476 \\
Llama-3.1-8B & 32 & IFEval & score & 0.303 & \textbf{0.315} & 0.311 & 0.307 & 0.224 \\
Llama-3.1-8B & 32 & CSQA & acc & 0.740 & 0.735 & 0.737 & 0.742 & \textbf{0.785} \\
\addlinespace
Llama-3.1-8B & 64 & GSM8K & acc & 0.659 & \textbf{0.661} & 0.654 & 0.657 & 0.621 \\
Llama-3.1-8B & 64 & HumanEval & pass@1 & 0.488 & 0.482 & 0.488 & \textbf{0.506} & 0.476 \\
Llama-3.1-8B & 64 & IFEval & score & 0.312 & 0.311 & \textbf{0.317} & 0.308 & 0.230 \\
Llama-3.1-8B & 64 & CSQA & acc & 0.740 & 0.734 & 0.738 & 0.740 & \textbf{0.782} \\
\addlinespace
Llama-3.1-8B & 128 & GSM8K & acc & 0.657 & 0.659 & \textbf{0.668} & 0.661 & 0.614 \\
Llama-3.1-8B & 128 & HumanEval & pass@1 & 0.488 & 0.488 & \textbf{0.494} & 0.488 & 0.476 \\
Llama-3.1-8B & 128 & IFEval & score & 0.305 & \textbf{0.321} & 0.312 & 0.306 & 0.223 \\
Llama-3.1-8B & 128 & CSQA & acc & 0.740 & 0.736 & 0.735 & 0.743 & \textbf{0.784} \\
\addlinespace
Llama-3.1-8B & 256 & GSM8K & acc & 0.655 & 0.657 & 0.659 & \textbf{0.660} & 0.610 \\
Llama-3.1-8B & 256 & HumanEval & pass@1 & \textbf{0.494} & 0.488 & \textbf{0.494} & 0.476 & 0.470 \\
Llama-3.1-8B & 256 & IFEval & score & 0.305 & 0.312 & \textbf{0.323} & 0.314 & 0.218 \\
Llama-3.1-8B & 256 & CSQA & acc & 0.741 & 0.740 & 0.737 & 0.740 & \textbf{0.783} \\
\midrule
Qwen3-8B & 32 & GSM8K & acc & 0.809 & 0.801 & 0.807 & 0.811 & \textbf{0.814} \\
Qwen3-8B & 32 & HumanEval & pass@1 & 0.488 & 0.512 & 0.500 & 0.494 & \textbf{0.530} \\
Qwen3-8B & 32 & IFEval & score & 0.590 & 0.525 & 0.534 & \textbf{0.603} & 0.179 \\
Qwen3-8B & 32 & CSQA & acc & 0.852 & 0.852 & 0.851 & 0.853 & \textbf{0.855} \\
\addlinespace
Qwen3-8B & 64 & GSM8K & acc & 0.807 & 0.806 & 0.805 & 0.810 & \textbf{0.811} \\
Qwen3-8B & 64 & HumanEval & pass@1 & 0.494 & 0.482 & \textbf{0.506} & 0.488 & \textbf{0.506} \\
Qwen3-8B & 64 & IFEval & score & 0.582 & 0.535 & 0.543 & \textbf{0.598} & 0.181 \\
Qwen3-8B & 64 & CSQA & acc & 0.848 & 0.851 & 0.851 & 0.853 & \textbf{0.855} \\
\addlinespace
Qwen3-8B & 128 & GSM8K & acc & 0.815 & 0.805 & 0.802 & 0.810 & \textbf{0.816} \\
Qwen3-8B & 128 & HumanEval & pass@1 & 0.488 & 0.506 & 0.506 & 0.494 & \textbf{0.512} \\
Qwen3-8B & 128 & IFEval & score & 0.590 & 0.535 & 0.552 & \textbf{0.597} & 0.173 \\
Qwen3-8B & 128 & CSQA & acc & \textbf{0.855} & 0.852 & 0.851 & 0.852 & 0.853 \\
\addlinespace
Qwen3-8B & 256 & GSM8K & acc & 0.808 & 0.805 & 0.801 & 0.805 & \textbf{0.817} \\
Qwen3-8B & 256 & HumanEval & pass@1 & 0.494 & \textbf{0.500} & 0.488 & 0.494 & \textbf{0.500} \\
Qwen3-8B & 256 & IFEval & score & 0.588 & 0.523 & 0.547 & \textbf{0.604} & 0.169 \\
Qwen3-8B & 256 & CSQA & acc & \textbf{0.855} & 0.853 & 0.850 & 0.852 & 0.853 \\
\bottomrule
\end{tabular}
\caption{Main results on \textbf{Llama-3.1-8B} and \textbf{Qwen3-8B} using \textbf{LoRA} adapters. \textbf{Calibration Size} denotes \texttt{calib\_samples}. \textbf{Baseline} denotes the unedited adapter (\texttt{unedited}). Boldface marks the best among baseline vs edited policies within each row.\lz{这个结果表是想呈现什么样的一个结论？重新组织一下？不知道你想表达什么，而且不一定要全塞在一个表格里？感觉这个表里的有些结果或者实验没什么用处？这个表格实在是太混乱了，先想一下你想表达什么}}
\label{tab:main_results_llama_qwen_lora}
\end{table*}

\begin{table*}[t]
\centering
\small
\begin{tabular}{l c l l c c c c c}
\toprule
\textbf{Model} & \textbf{Calib} & \textbf{Task} & \textbf{Metric} &
\textbf{Baseline} & \textbf{abs\_select} & \textbf{smooth\_abs} & \textbf{random\_index} & \textbf{grad\_direction} \\
\midrule
Llama-3.1-8B & 32 & GSM8K & acc & \textbf{0.666} & \textbf{0.666} & 0.661 & 0.663 & 0.615 \\
Llama-3.1-8B & 32 & HumanEval & pass@1 & \textbf{0.482} & \textbf{0.482} & \textbf{0.482} & 0.476 & \textbf{0.482} \\
Llama-3.1-8B & 32 & IFEval & score & 0.317 & \textbf{0.320} & 0.311 & 0.314 & 0.186 \\
Llama-3.1-8B & 32 & CSQA & acc & 0.740 & 0.726 & 0.727 & 0.742 & \textbf{0.785} \\
\addlinespace
Llama-3.1-8B & 64 & GSM8K & acc & \textbf{0.666} & 0.660 & 0.662 & 0.661 & 0.623 \\
Llama-3.1-8B & 64 & HumanEval & pass@1 & \textbf{0.488} & 0.476 & 0.470 & \textbf{0.488} & 0.476 \\
Llama-3.1-8B & 64 & IFEval & score & 0.314 & 0.315 & \textbf{0.318} & 0.317 & 0.187 \\
Llama-3.1-8B & 64 & CSQA & acc & 0.742 & 0.727 & 0.723 & 0.742 & \textbf{0.783} \\
\addlinespace
Llama-3.1-8B & 128 & GSM8K & acc & 0.659 & \textbf{0.664} & 0.662 & 0.650 & 0.621 \\
Llama-3.1-8B & 128 & HumanEval & pass@1 & \textbf{0.500} & 0.482 & 0.488 & \textbf{0.500} & 0.470 \\
Llama-3.1-8B & 128 & IFEval & score & \textbf{0.315} & 0.309 & 0.312 & 0.314 & 0.189 \\
Llama-3.1-8B & 128 & CSQA & acc & 0.740 & 0.727 & 0.725 & 0.740 & \textbf{0.782} \\
\addlinespace
Llama-3.1-8B & 256 & GSM8K & acc & 0.659 & \textbf{0.667} & 0.665 & 0.656 & 0.625 \\
Llama-3.1-8B & 256 & HumanEval & pass@1 & 0.500 & 0.482 & 0.482 & \textbf{0.506} & 0.494 \\
Llama-3.1-8B & 256 & IFEval & score & 0.314 & 0.317 & \textbf{0.321} & 0.317 & 0.193 \\
Llama-3.1-8B & 256 & CSQA & acc & 0.740 & 0.731 & 0.728 & 0.744 & \textbf{0.783} \\
\midrule
Qwen3-8B & 32 & GSM8K & acc & 0.806 & \textbf{0.807} & \textbf{0.807} & \textbf{0.807} & 0.788 \\
Qwen3-8B & 32 & HumanEval & pass@1 & 0.482 & 0.494 & \textbf{0.506} & 0.482 & 0.482 \\
Qwen3-8B & 32 & IFEval & score & 0.584 & 0.478 & 0.490 & \textbf{0.608} & 0.017 \\
Qwen3-8B & 32 & CSQA & acc & 0.852 & 0.844 & 0.850 & \textbf{0.853} & 0.838 \\
\addlinespace
Qwen3-8B & 64 & GSM8K & acc & 0.806 & 0.806 & 0.807 & \textbf{0.808} & 0.802 \\
Qwen3-8B & 64 & HumanEval & pass@1 & 0.476 & 0.488 & 0.488 & \textbf{0.500} & 0.482 \\
Qwen3-8B & 64 & IFEval & score & 0.594 & 0.481 & 0.478 & \textbf{0.610} & 0.014 \\
Qwen3-8B & 64 & CSQA & acc & 0.852 & 0.848 & 0.848 & \textbf{0.853} & 0.841 \\
\addlinespace
Qwen3-8B & 128 & GSM8K & acc & \textbf{0.819} & 0.802 & 0.807 & 0.807 & 0.798 \\
Qwen3-8B & 128 & HumanEval & pass@1 & 0.482 & 0.476 & 0.482 & \textbf{0.488} & 0.476 \\
Qwen3-8B & 128 & IFEval & score & 0.586 & 0.488 & 0.478 & \textbf{0.606} & 0.014 \\
Qwen3-8B & 128 & CSQA & acc & 0.850 & \textbf{0.853} & 0.847 & 0.850 & 0.839 \\
\addlinespace
Qwen3-8B & 256 & GSM8K & acc & 0.806 & \textbf{0.812} & 0.803 & 0.811 & 0.797 \\
Qwen3-8B & 256 & HumanEval & pass@1 & 0.476 & 0.482 & 0.494 & \textbf{0.500} & 0.470 \\
Qwen3-8B & 256 & IFEval & score & 0.583 & 0.484 & 0.486 & \textbf{0.604} & 0.016 \\
Qwen3-8B & 256 & CSQA & acc & 0.849 & 0.848 & \textbf{0.853} & \textbf{0.853} & 0.835 \\
\bottomrule
\end{tabular}
\caption{Main results on \textbf{Llama-3.1-8B} and \textbf{Qwen3-8B} using \textbf{LoRA} adapters with \texttt{preserve\_energy=None}. \textbf{Calib} denotes \texttt{calib\_samples}. \textbf{Baseline} denotes the unedited adapter (\texttt{unedited}). Boldface marks the best among baseline vs edited policies within each row.}
\label{tab:main_results_llama_qwen_lora_pe_none}
\end{table*}

\begin{table*}[t]
\centering
\small
\begin{tabular}{l c l l c c c c c}
\toprule
\textbf{Model} & \textbf{Calib} & \textbf{Task} & \textbf{Metric} &
\textbf{Baseline} & \textbf{abs\_select} & \textbf{smooth\_abs} & \textbf{random\_index} & \textbf{grad\_direction} \\
\midrule
Llama-3.1-8B & 128 & GSM8K & acc & 0.658 & \textbf{0.666} & \textbf{0.666} & 0.650 & 0.637 \\
Llama-3.1-8B & 128 & HumanEval & pass@1 & \textbf{0.500} & 0.482 & 0.488 & 0.488 & 0.470 \\
Llama-3.1-8B & 128 & IFEval & score & 0.312 & 0.315 & 0.312 & 0.308 & \textbf{0.317} \\
Llama-3.1-8B & 128 & CSQA & acc & 0.741 & 0.743 & 0.740 & 0.742 & \textbf{0.744} \\
\midrule
Qwen3-8B & 128 & GSM8K & acc & \textbf{0.819} & 0.802 & 0.807 & 0.810 & 0.809 \\
Qwen3-8B & 128 & HumanEval & pass@1 & 0.476 & \textbf{0.500} & 0.494 & \textbf{0.500} & \textbf{0.512} \\
Qwen3-8B & 128 & IFEval & score & \textbf{0.585} & 0.566 & 0.565 & 0.572 & 0.499 \\
Qwen3-8B & 128 & CSQA & acc & 0.849 & 0.851 & 0.854 & 0.852 & \textbf{0.857} \\
\bottomrule
\end{tabular}
\caption{Editing \textbf{attention input projections} (\texttt{q\_proj}, \texttt{k\_proj}, \texttt{v\_proj}) with \texttt{calib\_samples=128} and \texttt{preserve\_energy=l1}. \textbf{Baseline} is the unedited adapter; boldface marks the best among baseline and edited policies for each row.}
\label{tab:attn_inputs_qkv_l1_calib128}
\end{table*}


\begin{table*}[t]
\centering
\small
\begin{tabular}{l c l l c c c c c}
\toprule
\textbf{Model} & \textbf{Calib} & \textbf{Task} & \textbf{Metric} &
\textbf{Baseline} & \textbf{abs\_select} & \textbf{smooth\_abs} & \textbf{random\_index} & \textbf{grad\_direction} \\
\midrule
Llama-3.1-8B & 128 & GSM8K & acc &
0.658 & 0.660 & \textbf{0.662} & 0.660 & 0.538 \\
Llama-3.1-8B & 128 & HumanEval & pass@1 &
\textbf{0.506} & 0.457 & 0.463 & 0.494 & 0.476 \\
Llama-3.1-8B & 128 & IFEval & score &
0.313 & 0.311 & \textbf{0.315} & 0.314 & 0.195 \\
Llama-3.1-8B & 128 & CSQA & acc &
0.742 & 0.690 & 0.699 & 0.742 & \textbf{0.790} \\
\midrule
Qwen3-8B & 128 & GSM8K & acc &
0.814 & 0.802 & 0.798 & \textbf{0.818} & 0.778 \\
Qwen3-8B & 128 & HumanEval & pass@1 &
0.482 & 0.488 & 0.494 & 0.482 & \textbf{0.524} \\
Qwen3-8B & 128 & IFEval & score &
\textbf{0.594} & 0.511 & 0.524 & 0.582 & 0.071 \\
Qwen3-8B & 128 & CSQA & acc &
\textbf{0.852} & \textbf{0.852} & \textbf{0.852} & \textbf{0.852} & 0.846 \\
\bottomrule
\end{tabular}
\caption{Results when editing \textbf{all modules} (\texttt{down\_proj}, \texttt{o\_proj}, \texttt{q\_proj}, \texttt{k\_proj}, \texttt{v\_proj}, \texttt{up\_proj}, \texttt{gate\_proj}) with \texttt{preserve\_energy=l1} and \texttt{calib\_samples=128}. \textbf{Baseline} denotes the unedited adapter (\texttt{unedited}); boldface marks the best among baseline vs edited policies within each row.}
\label{tab:all_modules_l1_calib128}
\end{table*}


\begin{table*}[t]
\centering
\small
\begin{tabular}{l c l l c c c c c}
\toprule
\textbf{Model} & \textbf{Calib} & \textbf{Task} & \textbf{Metric} &
\textbf{Baseline} & \textbf{abs\_select} & \textbf{smooth\_abs} & \textbf{random\_index} & \textbf{grad\_direction} \\
\midrule
Llama-3.1-8B & 128 & GSM8K & acc &
\textbf{0.663} & 0.658 & 0.659 & 0.659 & 0.592 \\
Llama-3.1-8B & 128 & HumanEval & pass@1 &
\textbf{0.500} & 0.476 & 0.470 & 0.482 & 0.451 \\
Llama-3.1-8B & 128 & IFEval & score &
\textbf{0.313} & 0.299 & 0.303 & \textbf{0.313} & 0.205 \\
Llama-3.1-8B & 128 & CSQA & acc &
0.741 & 0.696 & 0.710 & 0.740 & \textbf{0.787} \\
\midrule
Qwen3-8B & 128 & GSM8K & acc &
0.805 & 0.806 & 0.803 & \textbf{0.817} & 0.789 \\
Qwen3-8B & 128 & HumanEval & pass@1 &
0.482 & 0.457 & 0.488 & 0.506 & \textbf{0.567} \\
Qwen3-8B & 128 & IFEval & score &
\textbf{0.583} & 0.574 & \textbf{0.583} & 0.579 & 0.462 \\
Qwen3-8B & 128 & CSQA & acc &
\textbf{0.852} & \textbf{0.852} & 0.850 & 0.849 & 0.851 \\
\bottomrule
\end{tabular}
\caption{Results when editing \textbf{MLP internal modules} (\texttt{up\_proj}, \texttt{gate\_proj}) with \texttt{preserve\_energy=l1} and \texttt{calib\_samples=128}. \textbf{Baseline} denotes the unedited adapter (\texttt{unedited}); boldface marks the best among baseline vs edited policies within each row.}
\label{tab:up_gate_l1_calib128}
\end{table*}

